Project-Level Encoding for Neural Source Code Summarization of Subroutines

Source code summarization of a subroutine is the task of writing a short, natural language description of that subroutine. The description usually serves in documentation aimed at programmers, where even brief phrase (e.g. "compresses data to a zip file") can help readers rapidly comprehend what a subroutine does without resorting to reading the code itself. Techniques based on neural networks (and encoder-decoder model designs in particular) have established themselves as the state-of-the-art. Yet a problem widely recognized with these models is that they assume the information needed to create a summary is present within the code being summarized itself - an assumption which is at odds with program comprehension literature. Thus a current research frontier lies in the question of encoding source code context into neural models of summarization. In this paper, we present a project-level encoder to improve models of code summarization. By project-level, we mean that we create a vectorized representation of selected code files in a software project, and use that representation to augment the encoder of state-of-the-art neural code summarization techniques. We demonstrate how our encoder improves several existing models, and provide guidelines for maximizing improvement while controlling time and resource costs in model size.

==> rqfivetbl.tex <==
\begin{figure}[!h]
	\centering
	\small
	\vspace{-0.2cm}
	\begin{tabular}{lllllll}
		& \multicolumn{1}{r}{BLEU:}             & \multicolumn{1}{c}{A} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4}      \\
		\multirow{3}{*}{} & \multicolumn{1}{l|}{attendgru-pc}    & 00.00                 & 00.00                 & 00.00                 & 00.00                 & \multicolumn{1}{l}{00.00} \\
		& \multicolumn{1}{l|}{attendgru-pc-A1} & 00.00                 & 00.00                 & 00.00                 & 00.00                 & \multicolumn{1}{l}{00.00} \\
		& \multicolumn{1}{l|}{attendgru-pc-A2} & 00.00                 & 00.00                 & 00.00                 & 00.00                 & \multicolumn{1}{l}{00.00}
	\end{tabular}
	\vspace{-0.2cm}
\end{figure}
